Noise limits for dc SQUID readout of high-$Q$ resonators below 300 MHz

We present the limits on noise for the readout of cryogenic high-$Q$ resonators using dc Superconducting Quantum Interference Devices (SQUIDs) below 300 MHz. This analysis uses realized first-stage SQUIDs (previously published), whose performance is well described by Tesche-Clarke (TC) theory, coupled directly to the resonators. We also present data from a prototype second-stage dc SQUID array designed to couple to this first-stage SQUID as a follow-on amplifier with high system bandwidth. This analysis is the first full consideration of dc SQUID noise performance referred to a high-$Q$ resonator over this frequency range, and is presented relative to the standard quantum limit. We include imprecision, backaction, and backaction-imprecision noise correlations from TC theory, the noise contributed by the second-stage SQUIDs, wiring, and preamplifiers, and optimizations for both on-resonance measurements and off-resonance scan sensitivity. This architecture has modern relevance due to the increased interest in axion searches and the requirements of the DMRadio-m$^3$ axion search, which will use dc SQUIDs in this frequency range.

==> authors_erdos.tex <==
\author{Macska~Erdös}
\affiliation{Department of Physics, Stanford University, Stanford, CA 94305}
\affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA 94305}

% \author{T.~Ankel}
% \affiliation{Department of Physics, Stanford University, Stanford, CA 94305}
% \affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA 94305}

% \author{C.~Bartram}
% \affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025}
% \affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA 94305}

% \author{J.~N.~Benabou}
% \affiliation{Berkeley Center for Theoretical Physics, University of California, Berkeley, CA 94720, U.S.A.}
% \affiliation{Theoretical Physics Group, Lawrence Berkeley National Laboratory, Berkeley, CA 94720, U.S.A.}

% \author{L.~Brouwer}
% \affiliation{Accelerator Techology and Applied Physics Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720}

% \author{S.~Chaudhuri}
% \affiliation{Department of Physics, Princeton University, Princeton, NJ 08544}

% \author{H.~-M.~Cho}
% \affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025}
% \affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA 94305}

% \author{J.~Corbin}
% \affiliation{Department of Physics, Stanford University, Stanford, CA 94305}
% \affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA 94305}

% \author{W.~Craddock}
% \affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025}

% \author{A.~Droster}
% \affiliation{Department of Nuclear Engineering, University of California, Berkeley, Berkeley, CA 94720}

% \author{J.~W.~Foster}
% \affiliation{Center for Theoretical Physics, Massachusetts Institute of Technology, Cambridge, MA 02139}

% \author{J.~T.~Fry}
% \affiliation{Laboratory of Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA 02139}

% \author{P.~W.~Graham}
% \affiliation{Department of Physics, Stanford University, Stanford, CA 94305}

% \author{R.~Henning}
% \affiliation{Department of Physics and Astronomy, University of North Carolina, Chapel Hill, Chapel Hill, North Carolina, 27599}
% \affiliation{Triangle Universities Nuclear Laboratory, Durham, NC 27710}

% \author{K.~D.~Irwin}
% \email{irwin@stanford.edu}
% \affiliation{Department of Physics, Stanford University, Stanford, CA 94305}
% \affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025}
% \affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA 94305}

% \author{A.~Keller}
% \affiliation{Department of Nuclear Engineering, University of California, Berkeley, Berkeley, CA 94720}

% \author{R.~Kolevatov}
% \affiliation{Department of Physics, Princeton University, Princeton, NJ 08544}

% \author{A.~Kunder}
% \affiliation{Department of Physics, Stanford University, Stanford, CA 94305}
% \affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA 94305}

% \author{N.~Kurita}
% \affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025}

% \author{A.~F.~Leder}
% \affiliation{Department of Nuclear Engineering, University of California, Berkeley, Berkeley, CA 94720}
% \affiliation{Physics Division, Lawrence Berkeley National Laboratory, Berkeley, CA 94720}

% \author{D.~Li}
% \affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025}
% \affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA 94305}

% \author{J.~L.~Ouellet}
% \affiliation{Laboratory of Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA 02139}

% \author{K.~M.~W.~Pappas}
% \affiliation{Laboratory of Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA 02139}

% \author{N.~M.~Rapidis}
% \affiliation{Department of Physics, Stanford University, Stanford, CA 94305}
% \affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA 94305}

% \author{C.~P.~Salemi}
% \email{salemi@stanford.edu}
% \affiliation{Department of Physics, Stanford University, Stanford, CA 94305}
% \affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025}
% \affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA 94305}

% \author{M.~Simanovskaia}
% \affiliation{Department of Physics, Stanford University, Stanford, CA 94305}
% \affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA 94305}

% \author{J.~Singh}
% \affiliation{Department of Physics, Stanford University, Stanford, CA 94305}
% \affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA 94305}

% \author{E.~C.~van~Assendelft}
% \affiliation{Department of Physics, Stanford University, Stanford, CA 94305}
% \affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA 94305}

% \author{K.~van~Bibber}
% \affiliation{Department of Nuclear Engineering, University of California, Berkeley, Berkeley, CA 94720}

% \author{K.~Wells}
% \affiliation{Department of Physics, Stanford University, Stanford, CA 94305}

% \author{L.~Winslow}
% \affiliation{Laboratory of Nuclear Science, Massachusetts Institute of Technology, Cambridge, MA 02139}

% \author{W.~J.~Wisniewski}
% \affiliation{SLAC National Accelerator Laboratory, Menlo Park, CA 94025}

% \author{D.~Wright}
% \affiliation{Department of Physics, Stanford University, Stanford, CA 94305}
% \affiliation{Kavli Institute for Particle Astrophysics and Cosmology, Stanford University, Stanford, CA 94305}

% \author{B.~A.~Young}
% \affiliation{Department of Physics, Santa Clara University, Santa Clara, CA 95053}

